Callisto: Entropy based test generation and data quality assessment for Machine Learning Systems

Machine Learning (ML) has seen massive progress in the last decade and as a result, there is a pressing need for validating ML-based systems. To this end, we propose, design and evaluate CALLISTO - a novel test generation and data quality assessment framework. To the best of our knowledge, CALLISTO is the first blackbox framework to leverage the uncertainty in the prediction and systematically generate new test cases for ML classifiers. Our evaluation of CALLISTO on four real world data sets reveals thousands of errors. We also show that leveraging the uncertainty in prediction can increase the number of erroneous test cases up to a factor of 20, as compared to when no such knowledge is used for testing. CALLISTO has the capability to detect low quality data in the datasets that may contain mislabelled data. We conduct and present an extensive user study to validate the results of CALLISTO on identifying low quality data from four state-of-the-art real world datasets.

==> motivation.tex <==
%\section{Motivation}
%\label{sec:motivation}
%
%To further elucidate our motivation to research this technique, we 
%sketch two situations that are we think are likely to occur in the future.  
%We also show these problems that may crop up because of the widespread 
%proliferation of ML and then we sketch a sample solution that uses our 
%\MLT technique to solve these problems. 
%
%%\smallskip
%%\noindent
%%\textbf{Testing ML Systems:} It is easy to see that the success of ML is
%%critically dependent on our ability to collect and annotate data. As 
%%we move towards more and more sophisticated techniques and tools for 
%%data collection, we'll need to update our toolkit for data management as 
%%well. A critical part of this ML pipeline remains the testing of models 
%%produced.
%%
%%%Regression testing involves the re-running of tests to ensure that software
%%%that was developed previously still performs after changes
%%%\cite{testing-book}. In the context for ML, the change is new, annotated
%%%data that is added to the training data and the new ML model developed from 
%%%that. Additionally, the regression tests is the previous testing data. 
%%
%%The rate of growth of data is massive as we have come to see in recent 
%%years. If we assume a conservative rate of growth of 30\% per iteration
%%of change in the ML model \revise{is iteration the right word here?}. 
%%For a starting set of 1,000,000 data points, this grows to $\approx$
%%50 billion data points in 50 iterations. The computational costs
%%of running tests on all these data points is massive. We aim to 
%%reduce the size of the testing needed, but retain the efficacy with \MLT. 
%%
%%%A significant reduction in
%%%the set of regression tests could lead to massive improvements in 
%%%turn around times for this data pipeline. 
%%
%%We envision that the user shall use our \MLT tool to build a set of 
%%tests which are most effective to expose the faults of the model.
%%In addition to this, \MLT will also assist the users to expose data
%%that is of low quality and potentially mislabelled. 
%
%
%%These sets
%%will consist of the inputs that are most likely to show faults in the ML
%%model. Additionally, these sets will be much smaller than the original 
%%dataset, resulting in massive savings in time and compute costs.
%
%\smallskip
%\noindent
%\textbf{Test Generation:} Test generation in ML presents a unique software 
%engineering challenge. The goal of test generation is to discover 
%erroneous behaviours in the software under test. In the context of ML, 
%there have been various techniques that have been proposed such as
%such as differential testing~\cite{deeepxplore}, metamorphic 
%testing~\cite{deeptest}\cite{deeproad}, concolic 
%testing~\cite{deepconcolic}, model 
%mutation~\cite{advSampleDetection} and probabilistic 
%search~\cite{aequitas}. 
%
%In our work, we want to build a cohesive framework to aid all of these
%techniques. Namely, we want \MLT to make test generation even better.
%If we consider the example presented before, it is easy to see that 
%applying these test generation techniques to all the inputs is very time
%consuming. In a well trained ML model, the error rate 
%might be low and running all tests may be unnecessary.
%
%\begin{figure}[h]
%\begin{center}
%\includegraphics[scale=1.1]{figs/test-gen-intuition.pdf}
%\end{center}
%\caption{Test \MLT intuition}
%\label{fig:test-gen-intuition}
%\end{figure}
%
%Assuming the test framework only runs three metamorphic tests, 
%a na\"{i}ve 
%approach will have to eventually run $\approx$150 billion tests. This is 
%clearly untenable in the long run. We use \MLT to identify inputs which 
%are prone to causing errors. This set is usually much smaller than 
%the full dataset and will exhibit highly erroneous behaviour. 
%
%A user can employ the \MLT technique to quickly and efficiently identify 
%which inputs to choose for further perturbation. This will aid the user 
%to discover erroneous behaviours without extensive testing of the entire 
%dataset. 
%
%We illustrate the intuition behind \MLT's test generation in approach in 
%\Cref{fig:test-gen-intuition}. Consider a metamorphic transformation $M$
%and inputs $A_1, A_2 $ and $A$. A rudimentary approach would 
%apply $M$ to all the data points leading to large computational 
%overheads. \MLT aims to discover points like $A$ which will allow users 
%to selectively apply a metamorphic relation to inputs which are likely
%to cause errors. \MLT will avoid points such as $A_1$ and $A_2$.
%
%\begin{figure*}[h]
%\begin{center}
%\begin{tabular}{cc}
%\includegraphics[scale=0.12]{figs/Motivation-1.pdf} & 
%\includegraphics[scale=0.12]{figs/Motivation-2.pdf} \\
%{\bf (a)} & {\bf (b)} 
%\end{tabular}
%\end{center}
%\vspace*{-0.15in}
%\caption{}
%\label{fig:motivation-workings}
%\end{figure*}
%
%\smallskip
%\noindent
%\textbf{Data Quality:} As the amount of data increases exponentially, a
%related problem of data quality will present itself. As more and more 
%data is generated and labelled automatically, the problem is to identify 
%the cases where the automatic data generation and/or labelling failed and 
%is likely of low quality. 
%
%The obvious and na\"{i}ve  approach is to engage humans to verify the data. 
%The cost of this can be very high and recurring as the amount of data 
%generated increases. 
%
%Our \MLT approach aims to flag these mislabelled and/or low quality inputs 
%for further intervention. The size of these flagged sets should be 
%significantly smaller in comparison to the full dataset and the cost of 
%human intervention is much lesser. 
%
%This allows the data to be sanitised efficiently and will lead to
%building of high quality datasets with low computational overhead. 
%As a result, the quality of the models will also improve.
%
%\smallskip
%\noindent
%\textbf{Solution Sketch:} In a typical ML classifier, there is usually 
%a softmax layer~\cite{deeplearning-book}. This layer normalises the second
%last layer's output to a probability distribution of the number of output 
%classes. The class with the highest class is then the prediction.
%The higher the probability of that last layer, the more confident 
%the DNN is in that particular prediction. 
%
%We aim to leverage this output layer to make predictions about the data 
%point. To illustrate this, consider a data point $A$ with label $l_{2}$ 
%whose output vector is as shown below
%
%\begin{equation}
%\label{eqn:eg1}
%\begin{split}
%[l_{0}, ~l_{1}, ~l_{2}, ~l_{3}] \approx[0.033, 0.033, 0.99, 0.034]
%\end{split}
%\end{equation}
%
%\noindent
%and data point $B$ with label $l_{2}$ whose output vector is as shown 
%below
%
%\begin{equation}
%\label{eqn:eg2}
%\begin{split}
%[l_{0}, ~l_{1}, ~l_{2}, ~l_{3}] \approx[0.25, 0.2, 0.3, 0.25]
%\end{split}
%\end{equation}
%
%\noindent
%Intuitively, the quality of the prediction for input $B$, although correct 
%is worse because of the lack of high confidence. To capture this lack of 
%quality, we use Shannon Entropy~\cite{informationtheory-book} to quantify
%the diversity of the prediction. It is important to note that the Shannon 
%Index has been used as a popular measure of diversity in ecological 
%literature to quantify the diversity of a 
%population~\cite{shannon-ecology}. It is defined below
%
%\begin{equation}
%\label{eqn:shannon}
%\begin{split}
%H' = - \sum_{i=1}^{N} l_i \ln l_i
%\end{split}
%\end{equation}
%
%\noindent
%In \Cref{eqn:shannon}, $N$ are the number of labels and $l_i$ is the output
%of the Deep Neural Network for the $i^{th}$ label. 
%
%The $H'$ value for input $A$ is $\approx$ 0.35 and the $H'$ value for 
%input $B$ is $\approx$ 1.38. Thus, the higher the Shannon index 
%for an output the lower the quality of the output. 
%
%We use this to build test sets for ML models. The data points 
%which have a high Shannon index are the ones likely to be affected most 
%by input perturbations and/or metamorphic relations.
%
%For Test Generation, we capture the inputs like datapoint $B$ and use 
%those
%to test the ML classifier. Once we have these inputs we can use 
%metamorphic
%relations/perturbations to generate test examples efficiently. 
%
%Consider another data point $C$ with label $l_0$. Let this data point be 
%mislabelled with its true data point being $l_2$. It is inferred by the 
%model and the output is 
%
%\begin{equation}
%\label{eqn:eg3}
%\begin{split}
%[l_{0}, ~l_{1}, ~l_{2}, ~l_{3}] \approx[0.0033, 0.0033, 0.999, 0.0034]
%\end{split}
%\end{equation}
%
%The Shannon index for the out is $\approx$0.058. The ML model is very
%confident in the prediction. It is likely that such inputs are very low 
%in number, but it is nevertheless important to find these data points. 
%The idea is that these data points are the ones which are most likely 
%to be mislabelled. 
%
%
%
%
%
%
%
%
%
%
%  
%
%

